CO-BED: Information-Theoretic Contextual Optimization via Bayesian Experimental Design

We formalize the problem of contextual optimization through the lens of Bayesian experimental design and propose CO-BED -- a general, model-agnostic framework for designing contextual experiments using information-theoretic principles. After formulating a suitable information-based objective, we employ black-box variational methods to simultaneously estimate it and optimize the designs in a single stochastic gradient scheme. In addition, to accommodate discrete actions within our framework, we propose leveraging continuous relaxation schemes, which can naturally be integrated into our variational objective. As a result, CO-BED provides a general and automated solution to a wide range of contextual optimization problems. We illustrate its effectiveness in a number of experiments, where CO-BED demonstrates competitive performance even when compared to bespoke, model-specific alternatives.

==> problem_formulation.tex <==
\section{Problem Formulation}
%
\begin{figure}[t]
% \vspace{-20pt}
\centering
    \includegraphics[width=0.45\textwidth]{icml2023/figs/fig_illustrative.png}
    \vspace{-10pt}
    \caption{A stylized example. %scalar context $\rvc$ and a binary action $\rva \in \{A, B\}$.
    The dark (resp. light) shaded area shows our prior uncertainty about $y \mid \rva,\rvc$ arising from uncertainty in $\psi$, measured by one (resp. two) st.~dev.~from the mean.
    We want to select actions in experimental contexts $\rvc_1, \rvc_2, \rvc_3$ (orange dotted lines) whose outcomes will be most informative about~$\rvm^*$ (red cross) in the evaluation context $c^*$ (grey dashed line).
    % \vspace{-18pt}
    }
    \label{fig:stylized_example}
\end{figure}

\paragraph{Bayesian model.}
We assume that the relationship between contexts $\rvc \in \gC$, actions (or treatments or designs), $\rva \in \gA$, and rewards (or experimental outcomes), $y \in \R$ is modelled in a Bayesian manner, namely by specifying a prior probability distribution $p(\psi)$ on some (potentially infinitely-dimensional) parameter $\psi$, and a likelihood function (or simulator), $p(y \mid \capsi)$. 
%The likelihood can be explicit, i.e.~analytically available in closed form, or implicit, meaning we can draw samples $y \mid \capsi $, but the density is intractable. 
Different realizations of $\psi$ correspond to different hypotheses about the relationship between contexts, actions, and rewards, whilst marginalizing over $\psi$ summarizes the total Bayesian uncertainty in $y$ given $\rva$ and $\rvc$. 
The maximum achievable reward in a context $\rvc^{\prime}$ is given by $m(\rvc^{\prime}) = \E \left[ y \mid \rva_{\star},\rvc^{\prime} \right]$, where $\rva_{\star} = \arg\max_{\rva \in \gA} \E \left[ y \mid \rva, \rvc^{\prime} \right]$ is the optimal action. 
The \emph{regret} of some action $\rva^{\prime}$ is
\begin{equation}
    R\left(\rvc^{\prime}, \rva^{\prime}\right) = m\left(\rvc^{\prime}\right) - \E \left[ y \mid \rva^{\prime},\rvc^{\prime} \right].
    \label{eq:regret}
\end{equation}



% Despite the appealing properties of these approaches, adaptive data collection can often be infeasible to implement in practice due to engineering and infrastructure limitations, as well as the presence of delayed rewards~\cite{matsushima2020deployment,zanette2021design}. Furthermore, resources in real-world scenarios are limited, so we may wish to focus on extracting  maximum information from a given \emph{finite} budget.  
%A more viable alternative, therefore, could be to consider two distinct phases as in \citet{zanette2021design}: 

\paragraph{Experimentation and evaluation contexts.}
When designing experiments to collect data for some downstream task, we can distinguish between two phases: \emph{experimentation} and \emph{deployment}. In the experimentation phase, we collect a \emph{batch} of data by designing and applying actions to different contexts in parallel. The goal of this phase is not to maximize rewards but to learn about the underlying system. The data collected is then used to identify optimal context-specific decisions. These decisions are `rolled out' and kept fixed during the deployment phase, which aims to maximize rewards, so the success of a method is evaluated based on the regret~\eqref{eq:regret} in this second phase. 


\paragraph{Goal.} We aim to design a set of actions $\rvA = (\rva_1, \dots, \rva_D)$ to apply to a set of \emph{experimental contexts} $\rvC = (\rvc_1,\dots,\rvc_D)$ in order to efficiently learn about the max rewards $\rvm^* = (m(\rvc^*_1),\dots, m(\rvc^*_{D^*}))$ for a set of \emph{evaluation contexts} $\rvC^* = (\rvc^*_1,\dots,\rvc^*_{D^*})$.
The contexts $\rvC$ and $\rvC^*$ are fixed but arbitrary, so they can be the same or different from each other.
In the personalized marketing example, the experimental contexts $\rvC$ could represent the customers in a given city who will participate in a real-world experiment; the evaluation contexts $\rvC^*$, on the other hand, may represent the customers in a whole region where the campaign will be rolled out, and the updated model will be deployed. 

We emphasize that the goal of the design process in the experimentation phase is to obtain data that will aid in learning about the max rewards in the evaluation contexts, $\rvm^*$, rather than maximizing the rewards in the experimental contexts. 
This concept is illustrated in \cref{fig:stylized_example}, highlighting the distinction between the $\rvC$ and $\rvC^*$ in a stylized example involving two actions.
Whilst Action~A may lead to higher rewards in the experimental contexts, these rewards will be uninformative about the value of $\rvm^*$ since this action is apriori known to be suboptimal for the context of interest~$\rvc^*$.  

